Text2QR: Harmonizing Aesthetic Customization and Scanning Robustness for Text-Guided QR Code Generation

In the digital era, QR codes serve as a linchpin connecting virtual and physical realms. Their pervasive integration across various applications highlights the demand for aesthetically pleasing codes without compromised scannability. However, prevailing methods grapple with the intrinsic challenge of balancing customization and scannability. Notably, stable-diffusion models have ushered in an epoch of high-quality, customizable content generation. This paper introduces Text2QR, a pioneering approach leveraging these advancements to address a fundamental challenge: concurrently achieving user-defined aesthetics and scanning robustness. To ensure stable generation of aesthetic QR codes, we introduce the QR Aesthetic Blueprint (QAB) module, generating a blueprint image exerting control over the entire generation process. Subsequently, the Scannability Enhancing Latent Refinement (SELR) process refines the output iteratively in the latent space, enhancing scanning robustness. This approach harnesses the potent generation capabilities of stable-diffusion models, navigating the trade-off between image aesthetics and QR code scannability. Our experiments demonstrate the seamless fusion of visual appeal with the practical utility of aesthetic QR codes, markedly outperforming prior methods. Codes are available at \url{https://github.com/mulns/Text2QR}

==> figs/selr.tex <==

\setlength{\myfigwidth}{0.22\linewidth} % Adjust the size as needed
\begin{table}[h]
    \caption{Visualization of iterative refinement.}
    \label{tab:selr}
    \centering
    \begin{tabularx}{\linewidth}{>{\centering\arraybackslash}X *{4}{>{\centering\arraybackslash}X}}

    \toprule
    input (un-scannable) & iter=100 & iter=200 & iter=400 (scannable) \\
    \midrule

    % \includegraphics[width=\myfigwidth, height=\myfigwidth]{CVPR2024-T2QR/figs/refinement/01453/it000-e0538.jpg} & 
    % \includegraphics[width=\myfigwidth, height=\myfigwidth]{CVPR2024-T2QR/figs/refinement/01453/it100-e0029.jpg} & 
    % \includegraphics[width=\myfigwidth, height=\myfigwidth]{CVPR2024-T2QR/figs/refinement/01453/it200-e0025.jpg} & 
    % \includegraphics[width=\myfigwidth, height=\myfigwidth]{CVPR2024-T2QR/figs/refinement/01453/it400-e0014.jpg} \\

    
    \includegraphics[width=\myfigwidth, height=\myfigwidth]{CVPR2024-T2QR/figs/refinement/01705/it000-e0623.jpg} & 
    \includegraphics[width=\myfigwidth, height=\myfigwidth]{CVPR2024-T2QR/figs/refinement/01705/it100-e0057.jpg} & 
    \includegraphics[width=\myfigwidth, height=\myfigwidth]{CVPR2024-T2QR/figs/refinement/01705/it200-e0042.jpg} & 
    \includegraphics[width=\myfigwidth, height=\myfigwidth]{CVPR2024-T2QR/figs/refinement/01705/it400-e0032.jpg} \\

    
    \includegraphics[width=\myfigwidth, height=\myfigwidth]{CVPR2024-T2QR/figs/refinement/01742/it000-e0392.jpg} & 
    \includegraphics[width=\myfigwidth, height=\myfigwidth]{CVPR2024-T2QR/figs/refinement/01742/it100-e0009.jpg} & 
    \includegraphics[width=\myfigwidth, height=\myfigwidth]{CVPR2024-T2QR/figs/refinement/01742/it200-e0006.jpg} & 
    \includegraphics[width=\myfigwidth, height=\myfigwidth]{CVPR2024-T2QR/figs/refinement/01742/it400-e0011.jpg} \\

    
    \bottomrule
    \end{tabularx}

\end{table}
    
